How can I choose an explainer? An Application-grounded Evaluation of Post-hoc Explanations

There have been several research works proposing new Explainable AI (XAI) methods designed to generate model explanations having specific properties, or desiderata, such as fidelity, robustness, or human-interpretability. However, explanations are seldom evaluated based on their true practical impact on decision-making tasks. Without that assessment, explanations might be chosen that, in fact, hurt the overall performance of the combined system of ML model + end-users. This study aims to bridge this gap by proposing XAI Test, an application-grounded evaluation methodology tailored to isolate the impact of providing the end-user with different levels of information. We conducted an experiment following XAI Test to evaluate three popular post-hoc explanation methods -- LIME, SHAP, and TreeInterpreter -- on a real-world fraud detection task, with real data, a deployed ML model, and fraud analysts. During the experiment, we gradually increased the information provided to the fraud analysts in three stages: Data Only, i.e., just transaction data without access to model score nor explanations, Data + ML Model Score, and Data + ML Model Score + Explanations. Using strong statistical analysis, we show that, in general, these popular explainers have a worse impact than desired. Some of the conclusion highlights include: i) showing Data Only results in the highest decision accuracy and the slowest decision time among all variants tested, ii) all the explainers improve accuracy over the Data + ML Model Score variant but still result in lower accuracy when compared with Data Only; iii) LIME was the least preferred by users, probably due to its substantially lower variability of explanations from case to case.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> abs.tex <==
% OLD ABSTRACT

\iffalse
  % What is the problem?
  The recent \ac{XAI} push has had little impact on real-world decision-making systems. 
  The lack of rigor and authenticity on \ax{XAI} methods evaluation yields no guarantees on the tangible impact of showing an explanation to humans integrated in such systems (human-in-the-loop).
  % Why is the problem important?
  The deployment of \ac{XAI} methods based on unreliable assessments may inadvertently worsen the humans' performance and/or understanding of the task.
  
  % What is the solution?
  To address this, we propose an \ac{XAI} evaluation methodology that considers the different components involved in Human-AI cooperative systems: the data, the model, and the explanation method. Since each component represents increasing levels of information, the proposed methodology allows for more robust measurements of how each component affects human experts' decisions (e.g., time, accuracy, understanding). 
  
  We use Randomized controlled trials to conduct an unbiased \ac{XAI} evaluation experiment, where we isolate the effect of showing different explanations generated by different \ac{XAI} methods to a group of human experts. After measuring their effects on the humans' decision process, we apply statistical tests to detect significant differences between the methods and a control group (where no explanations were shown).
  %why is the solution important?
  Rather than measuring proxies of desiderata of explanations, the proposed methodology provides a rigorous perception of the actual usefulness (and impact) of different \ac{XAI} methods, thus promoting more informed decisions about their integration in real-world Human-AI decision-making systems.
  % Summary of contributions (including experimental results):
  The results of our experiment show that showing model scores decreases both performance and decision time, while showing explanations about the model decision increases performance, in general. 
  % We don't yet know what are the exact contributions. Maybe after seeing the results we can re-iterate this part.
\fi


  % What is the problem, and why is it important?
  The lack of consensus on the evaluation of \ac{XAI} methods difficults when comparing and choosing a method for a given task and end-users. This hinders the trust we have on the methods themselves, and consequently their use on high responsibility decision-making systems, where explanations can have a greater impact.
  % How can we solve it? 
  %We argue that the lack of studies where systematic application-grounded evaluations are employed cause the misalignment between recent strides and real-world usage on \ac{XAI}.
  
  % What do we do?
  In this work, we directly evaluate the effect of showing explanations on the efficiency of end-users in a decision-making task.
  This is done through randomized controlled trials where, we conduct an unbiased \ac{XAI} evaluation experiment, isolating the effect of showing different explanations generated by different methods to a group of human experts. After measuring their effects on task-specific performance metrics (e.g. accuracy), we apply statistical tests to detect significant differences between the methods and a control group (where no explanations were shown). %Additionally, we measure the effect of showing the score produced by the \ac{ML} model present at the decision-making system. 


% NEW ABSTRACT


There has been widespread interest in developing novel Explainable AI techniques to enhance transparency, trust and usability of algorithmic decision-making systems. However, there is a lack of adequate evaluation methodologies to assess the real impact of showing explanations to the end-users, i.e., the human-in-the-loop who interacts with the algorithm to make an informed decision. This study aims to bridge that gap by proposing an application-grounded evaluation methodology tailored to isolate the impact of providing different types of information to the end-user. This way we can reliable assess the usefulness of a given explanation method. 
%
We used the proposed methodology to conduct a user-study in a real-world application (payments fraud detection). Three fraud analysts reviewed a total of $1300$ real transactions using their day-to-day case management system. During the experiment, we gradually increased the information level in three stages: \textit{Data only}, \textit{Data + ML model score}, and \textit{Data + ML model score + Explanations}. Throughout the experiment, we monitor users' performance through accuracy, recall,false positive rate, and average review time. In later experiment stages, user feedback is also collected.
%
We find that showing explanations helped fraud analysts making faster decisions at the expense of decision accuracy. Therefore, popular \textit{posthoc} explanation methods do not seem to enhance end-user decision quality, indicating their limited usefulness and potential risks on high-stakes decision-making tasks.  
%We use the proposed methodology to run a user-study in a real-world fraud detection application to find whether \textit{post-hoc explanations promote better human performance in a fraud predictive task}. In our experiment, $3$ fraud analysts review a total of $1300$ transactions using their day-to-day review system. During the experiment, we gradually increase the information level in three stages (\textit{Data only}, \textit{Data + ML model}, and \textit{Data + ML model + Explainers}). Throughout the experiment, we monitor users' performance through accuracy, recall, \ac{FPR}, and average review time. In later experiment stages, user feedback is also collected.


%The black-box paradigm of machine learning paired with a stricter scrutiny of automated decision-making systems motivated a resurgence of \ac{XAI} methods. 

==> old_related_work.tex <==
\iffalse
\subsubsection{Intrinsic Evaluation}
\label{sssection:intrinsic_eval}

As previously mentioned, \textit{Intrinsic} evaluation refers to the evaluation through metrics or experiments that do not involve users. 
Evaluation methods in this category are usually reproducible because users do not partake in the collection of the evaluation metrics.
In this category, it is possible to find a subset of consistently applied metrics in the literature, such as fidelity or accuracy \cite{lakkaraju2016, shap:NIPS2017, plumb2020BBMInterpretability, tan2018learning, lundberg2019explainable, zhang2018top, guo18, ribeiro2016lime, zilke2016deepred, arras2019explaining, NIPS2018_7518, guidotti2018local, lakkaraju2019faithful, van2018contrastive}.

There were dedicated publications for novel techniques of intrinsic evaluation, introducing metrics such as Explicitness/Intelligibility (how easy are the explanations to understand), Faithfulness (how relevant is the explanation), Stability (how consistent are the explanations for similar instances) \cite{NIPS2018_8003}, Robustness (how stable are explanations for small perturbations) \cite{AlvarezMelis2018}.
%However, the rate of adoption of a metric does not necessarily mean they are applied properly and in a just manner.
%This is often the result of applying the metrics to measure the wrong aspects of explanation, instead of focusing on those that make up a good explanation method.

Also, some authors define custom metrics that are used to evaluate the new method and they rarely see use after that \cite{lakkaraju2016, lundberg2019explainable, guidotti2018local,lakkaraju2019faithful, van2018contrastive, NIPS2019_9264, mengnan19, zafar2019dlime}. For instance, the authors in \cite{lundberg2019explainable} uses 21 different intrinsic metrics (that basically measure the impact on the model); this practice can bring some ambiguity to the analysis of the evaluations, due to the lack of publications following the same methodology. Another example is the authors in \cite{NIPS2019_9264}, who measures the performance of the proposed explanation method by using Euclidean distance and Jaccard similarity. The authors in \cite{zafar2019dlime} also used Jaccard similarity, but with different purpose, measuring the stability of the explanations produced by the proposed method, comparing it to the state-of-the-art method LIME \cite{Ribeiro:2016}. In \cite{lakkaraju2016}, the authors define custom metrics (\textit{e.g.} \textit{average rule width} that measures the average number of predicates used in the explanation) to evaluate rule-based explanation methods, comparing the proposed method with others previously rule-based methods across three different datasets. Moreover, the authors in \cite{van2018contrastive} also propose a custom metric defined as time, that measures the average time the method takes to generate explanation for a given data point. 

Still in this category, it is possible to find some papers that resort to simulated users to run virtual user studies \cite{weerts2019casebased}. However, these are often criticized due to the impossibility to simulate real user feedback.

The main concern about the intrinsic evaluation is that it does not measure the impact of the explanations on the end user. It means that, although the explanation is faithful and stable, it may not improve the interpretability.


% Original paragraph for intrinsic evaluation
% Intrinsic evaluation consists on the evaluation through metrics or experiments where there are no users partaking on the method. 
% In this type of evaluation several metrics are consistent across publications but also many created or defined in the publication itself and are not used onward.

% Metrics like accuracy, fidelity and AUC ROC have been used through several works but there is cases where they do not evaluate the right characteristics that define a good explanation method.

% In this category, there is also some works that simulate users and perform "user studies", but since these are not real humans interacting with the system, there is the possible critic that these experiments are not capable of simulating real user feedback.
 
\subsubsection{Domain Knowledge Evaluation}
\label{sssection:domain_eval}

\textit{Domain knowledge} evaluation concerns the assessment of the explanation methods in their application domain. 
This includes the comparison of explanations against factors known to be the most important in a specific domain. 
Human experts in the different domains are responsible for the identification of key information. Ideally, the collected information identifies the experts own reasoning and explanations.
As an example, consider a credit card fraud setting. Fraud analysts have previously identified the time between consecutive transactions to be particularly instructive about transactions' legitimacy. 
Therefore, an explanation containing this information is more likely to be accepted as a good explanation. 

Naturally, it is not enough to have instructive explanations, they also have to make sense. 
They must reflect the context they occur on, \textit{i.e.}, an explanation that conveys the wrong information about a model's decision is of no use.  
Let us extend the fraud setting described previously. 
Suppose that a model confidently predicts a given transaction as suspicious because the time gap between consecutive transactions was a few milliseconds. 
A good explanation would correctly identify the time difference as a justification for the model's suspicious, whereas a defective explanation could point the shipping and billing names mismatch. 
While the latter carries important information for the fraud domain setting, it fails to identify the actual reason that justifies the model reasoning.

In the literature, this approach has been used to evaluate  multiple \ac{XAI} methods in different fields, including \ac{NLP}, finance, among others  \cite{alvarezmelis2017causal,guo2019exploring,NIPS2018_7340}. 
In the \ac{NLP} domain, \cite{alvarezmelis2017causal} use \ac{XAI} methods to explain black box predictors. 
To this end, they ask language experts to evaluate the quality of the explanations and examine their adequacy to explaining the model's decisions on a text translation task. 
% 2nd work
In another spectrum, \cite{guo2019exploring} applies an \ac{XAI} method to three datasets in different domains: meteorological data, energy production, and indoor temperature prediction. 
Given their variety, the authors elicited domain experts in the different fields to help selecting the most influential features. 
Then, the quality of the explanation method was simply measured by comparing its outputs against the previously collected features.  
% 3rd work
Also, \textit{domain knowledge} evaluation has been used in the fintech domain \cite{NIPS2018_7340}. \cite{NIPS2018_7340} focused on the evaluation of an \ac{XAI} method for a fraud risk prediction use case. The authors selected 45 instances (in their case, these represented invoices) and had both the \ac{XAI} method and the domain experts explaining them. 
Then, the authors determine the quality of the method's explanations by overlapping the two sets of explanations for each invoice and identifying possible matches.

Another recent evaluation in the fintech domain is that of \cite{collaris2018instancelevel}.
In this paper, the authors aim to test different \ac{XAI} methods applied to a Fraud Detection setting. 
They ask 5 domain experts to evaluate and validate the explanations retrieved by the different methods. 
To this end, they organize the explanations into two distinct dashboards. 
The first dashboard includes: (1) feature importance, \textit{i.e.}, how much each feature contributed for the model prediction, (2) partial dependence plot, \textit{i.e.}, the variation on the model predictions across feature values; and (3) the distribution of the training data and the instance being explained. 
On the other hand, the second dashboard contained a set of rule-based explanations that showed the model decision process. 
While no further details about the way the experiments were conducted are revealed, the authors claim that experts preferred rule-based explanations because they were more concise.
Furthermore, they conclude that the explanations retrieved by different \ac{XAI} methods are not consistent across methods, \textit{i.e.}, there are no guarantees that the most important features selected by one method match the ones selected by a different method. Finally, they argue that fraud experts still trusted the explanations, despite the exhibited inconsistency.

% Conclusion & Disadvantages
As a final remark, \textit{domain knowledge} approaches are capable of providing more qualitative measures of the performance of different \ac{XAI} techniques. 
Because they include a human component in the validation loop, the reported results are often perceived as more trustworthy. Plus, the high quality explanations are also assumed to resemble human-style explanations, for example by including the same information a human would when facing the same situation.  
In contrast, opponents of this type of evaluation often argue that this type of evaluation is often overlooked and that it does not take the human bias into account. 
Introducing the human in the evaluation loop is important because it provides valuable insights about the reasoning and the patterns that one would expect to find in a given domain. 
However, \ac{ML} models may learn patterns that are totally different from the ones learned by humans. 
In these cases, critics insist that \ac{XAI} methods might be unduly evaluated, since human evaluators tend to favor explanations matching their own reasoning. 
For example it might be the case that a given method is very good at explaining bad \ac{ML} models. 
Critics claim that the explainer will be given a worse appraisal because the explanations will, most likely, fail to match the expert's.

Once again, this discussion reflects the current lack of standardization in \ac{XAI} evaluation. 

\subsubsection{User Evaluation}
\label{sssection:user_eval}

In user-based evaluation, a group of people performs a task under different conditions.  
Selected participants may or may not have domain expertise in the area \cite{lakkaraju2016}, in which case they are randomly selected.

In general, during the experiment, participants are shown both the AI decisions and the corresponding explanations. 
In the end, participants fill a survey where they provide explicit feedback about the quality of the explanations \cite{lakkaraju2016, kulesza2013, narayanan2018humans, rader2018}. 
\cite{kulesza2013} included \textit{Likert} scales in their surveys in order to rate the quality of the explanation. 
In addition to explicit feedback, other works, like \cite{lakkaraju2016}, are also interested in collecting metrics based the user's footprint in the system, such as the accuracy and/or time to complete the task. 

User-based evaluation incorporates actual end-users in the evaluation stages and, for that reason, is capable of providing a more solid idea about the usefulness of the explanations.
Unfortunately, this strategy still lacks rigor.
Most drawn conclusions contain no statistical significance, for the authors do not perform statistical analysis to assess the explanations' effects on the accomplished tasks.

In a utilitarian perspective, many \ac{XAI} evaluation works focus on the collection of explicit feedback because it is the most direct for obtaining the users' perception on a given explanation. 
However, other measures, such as the time for concluding a task, can also be used as proxies for explanations' usefulness.

As a case in point, consider the evaluation of \textit{Precience}~\cite{Lundberg206540}, an \ac{ML}-based system that provides interpretable real-time predictions to help anaesthesiologists prevent hypoxemia during surgery.
To evaluate this system the authors use a two-fold approach. 
First, they apply \textit{domain knowledge} evaluation, where they compare the most important features given by the explanation method against the ones identified by the anaesthesiologists. 
Second, they resort to user testing and measure the different implicit feedback metrics, including the users' performance. 
To this end, they subject the users to two different experiments: one with the model explanations and other without any of those. 
This allowed the authors to isolate and quantify the impact of the explanations on the users' performance. 
It is noteworthy that the authors carried such a complete evaluation, involving both domain experts and the real-world end-users of the system. 
However, this evaluation is not sufficiently robust because the impacts of the \ac{ML} model alone were not properly disassociated from the explanations. 

Effectively, proper user testing of \ac{XAI} methods should consider all the following Human-AI configurations: (1) User-only, (2) User with the model decision; and (3) User with both the model decision and explanation. 
This aims to purposefully isolate the three interacting components in any Human-AI decision-making system - model, explanations, human. 
A careful analysis over the evaluation methodology carried on \textit{Precience} \cite{Lundberg206540} shows that only configurations (1) and (3) were considered. 
While this might reveal useful information, it is impossible to attribute the measured benefits to a single component (either the \ac{XAI} method or the \ac{ML} model).

As a different example of the application of user testing to \ac{XAI} evaluation, in \cite{weerts2019casebased} the authors explore a solution in a fraud detection setting. Their goal was to explain the decisions of an Human-AI decision-making system to domain experts. 
While, initially, the authors simulate user studies to estimate the ``coverage, precision, and trustworthiness'' of the explanations, they also conduct individual user studies through usability tests. 
They carry these tests using the ``think aloud'' protocol, \textit{i.e.}, a verbal protocol in which participants explain their reasoning aloud while performing the task. Additionally, the authors use \textit{Likert} scales to assess the explanations' perceived usefulness and ease of use.

In sum, if used properly, user-based evaluation is the most useful and trustworthy \ac{XAI} evaluation approaches. 
It accounts for the real-end impact that the \ac{XAI} methods may have in the Human-AI ecosystem they integrate. 
It quantifies the explanations' adequacy to a specific domain and also their practicality. 
Notwithstanding its potential, current state-of-the-art still reports biased and unsound results (e.g., weak statistical analysis, fail to isolate different interacting components). 
Up to this date, no studies or frameworks have tried to circumvent these limitations.
However, the need for a more robust and statistically sound methodology for carrying out \ac{XAI} user-based evaluation approaches is urgent. 
With different Human-AI decision-making systems being deployed every day, it is a question of time until end-users start demanding for useful, trustworthy, and effective explanations. 
\fi

==> old_table.tex <==
\begin{table*}[thbp]
  \captionsetup{width=.9\textwidth}
  \caption{
  Performance and time metrics for all variants of the experiment. Statistical significance is tested against the control group and between explanations.  
  $^{\star}$ indicates significant difference with control; $^{\blacklozenge}$ indicates significant difference with other explainers. Agreement metric is \textit{Fleiss' Kappa}.}
  \label{tab:metrics}

\begin{tabular}{c c c c c c c c}
    \hline
        \multirow{2}{*}{\textbf{Group}} & \multirow{2}{*}{\textbf{Explainer}} & \multirow{2}{*}{\textbf{Sample Size}} & \multicolumn{4}{c}{\textbf{Metrics}} & \multirow{2}{*}{\makecell{\textbf{Agreement}}} \\
    
    \cline{4-7}
     & & & \textbf{Accuracy (\%)} & \textbf{Recall (\%)} & \textbf{FPR (\%)} &  \textbf{Time (s)} \\
    \hline
   
       \makecell{Data only\\ (Control)}  & - & 200 & \makecell{\textbf{62.00}} & \makecell{\textbf{35.87}} & \makecell{15.74} & \makecell{59.50} & \makecell{0.41} \\
    
    \makecell{Data \\ + \\ Model Score} & - & 200 & \makecell{51.02$^{\star}$} & \makecell{25.00} & \makecell{19.57} &  \makecell{44.61$^{\star}$} & \makecell{-0.02} \\
    
     \multirow{4}{*}{\makecell{Data + \\ Model Score + \\ Explanations}} & LIME & 300 & \makecell{58.59} & \makecell{27.03} & \makecell{\textbf{10.07}} &  \makecell{50.29$^{\star}$} & \makecell{\textbf{0.53}} \\
    
      & TreeInterpreter & 300 & \makecell{56.52} & \makecell{25.55} & \makecell{12.67} &  \makecell{\textbf{43.03}$^{\star\blacklozenge}$} & \makecell{0.30} \\
     
    & TreeSHAP & 300 & \makecell{59.73} & \makecell{31.08} & \makecell{12.00} &  \makecell{45.72$^{\star}$} & \makecell{0.15} \\
    \hline
\end{tabular}
\end{table*}

%% OLD QUESTIONAIRE TABLE

\label{tab:Questionnaire}
\begin{tabular}{ m{4cm}  c}
  &  \multicolumn{1}{c}{\footnotesize \bfseries\parbox{0.14\textwidth}{Strongly\\ disagree}\parbox{0.06\textwidth}{\centering Strongly\\agree}} \tabularnewline
1) The explanation covered all the relevant information to help me make a decision.          & \parbox{0.20\textwidth}{\scaletable} \tabularnewline \vspace{0.2cm}
2) The explanation helped me decide faster.                                                  & \parbox{0.20\textwidth}{\scaletable} \tabularnewline \vspace{0.2cm}
3) The explanation was useful to help me make a decision.                                    & \parbox{0.20\textwidth}{\scaletable} \tabularnewline
\end{tabular}
